Distributed Error-Identification and Correction using Block-Sparse Optimization

The conventional solutions for fault-detection, identification, and reconstruction (FDIR) require centralized decision-making mechanisms which are typically combinatorial in their nature, necessitating the design of an efficient distributed FDIR mechanism that is suitable for multi-agent applications. To this end, we develop a general framework for efficiently reconstructing a sparse vector being observed over a sensor network via nonlinear measurements. The proposed framework is used to design a distributed multi-agent FDIR algorithm based on a combination of the sequential convex programming (SCP) and the alternating direction method of multipliers (ADMM) optimization approaches. The proposed distributed FDIR algorithm can process a variety of inter-agent measurements (including distances, bearings, relative velocities, and subtended angles between agents) to identify the faulty agents and recover their true states. The effectiveness of the proposed distributed multi-agent FDIR approach is demonstrated by considering a numerical example in which the inter-agent distances are used to identify the faulty agents in a multi-agent configuration, as well as reconstruct their error vectors.

==> sections/distributed/tikz_array.tex <==
\begin{center}
\begin{tikzpicture}[>=stealth,thick,baseline]
    
    \matrix [matrix of math nodes,left delimiter={[},right delimiter={]}](A){ 
    x_1(k)\\ x_2(k)\\ \vdots\\ x_{|\mathcal B|}(k)\\ \vdots \\ \phi(x_i(k),x_j(k))\\ \vdots \\
   };
    
    \begin{scope}[
    execute at begin node = $,
    execute at end node = $,
    ]
    \node[
     fit=(A-4-1)(A-4-1),
     inner xsep=28pt,inner ysep=0,
     label=left: h(x(k)) \coloneqq
    ](L) {};
    
  \node[
     fit=(A-6-1)(A-6-1),
     inner xsep=22pt,inner ysep=0,
     label={right, text=darkgray}: {(i,j) \in \mathcal E}
    ](L) {};
    \end{scope}
    
%   \node[
%      fit=(A-6-4)(A-6-4),
%      inner xsep=20pt,inner ysep=20pt,
%      label=below: $j$-ième colonne
%      ](C) {};

    \draw[->, darkgray](L.east)-- ([xshift=12pt]A-6-1.east);
    
    % \begin{scope}[decoration={square right brace, amplitude=6pt,raise=2pt}]
    % \draw[decorate,thick] (A-5-1.north east) -- (A-6-1.south east) node[midway,xshift=15pt]{text};
    % \end{scope}
    \draw[shorten >=2pt, shorten <=2pt, darkgray] ([xshift=81.5pt, yshift=-1pt]A-1-1.north east) --++(0:3mm)|-([xshift=78.5pt, yshift=3pt]A-4-1.south east) node[pos=.25, rotate=270, above]{\small $d|\mathcal B|$ entries};
    
        % \draw[shorten >=2pt, shorten <=2pt] ([xshift=70pt]A-5-1.north east) --++(0:3mm)|-([xshift=87pt]A-7-1.south east) node[pos=.25, rotate=270, above]{$m|\mathcal E|$ entries};
    \draw[shorten >=2pt, shorten <=2pt, darkgray] ([xshift=92pt, yshift=-2pt]A-5-1.north east) --++(0:3mm)|-([xshift=92pt, yshift=0pt]A-7-1.south east) node[pos=.25, rotate=270, above]{\small $m|\mathcal E|$ entries};

\end{tikzpicture}
\end{center}

==> sections/trashed.tex <==

When in the function $f(\bold v)$ in Theorem \ref{thm:proximal} we set $\bold A=\bold I$,
we get the proximal operator for $\|{}\cdot{}\|_2$, defined by:

\begin{align}
\textit{prox}_{\|{}\cdot{}\|_2}(\bold b) &= \argmin_{\bold v} \left(\frac{1}{2}\|\bold v - \bold b\|_2^2 + \|\bold v\|_2\right)\\&= \begin{cases}
\begin{array}{cl}
    \left(1- \frac{1}{\|\bold b\|_2}\right)\bold b &   \|\bold b\|_2 > 1\\
     \bold 0 &  \|\bold b\|_2 \leq 1
\end{array}
\end{cases}
\end{align}

which has an easier derivation by way of the Moreau decomposition. Our derivation additionally handles the cases of $\bold A$ being rank deficient, and is consistent with the proximal operator of $\|{}\cdot{}\|_2$ when $\bold A = \bold I$. More generally, we have the following corollaries, which are proved via substitution.

\begin{corollary}
If $\bold b$ is an eigenvector of $\bold A\bold A^T$ with eigenvalue $\lambda$, then the minimizer $\bold v^*$ of $f(\bold v)$ in Theorem \ref{thm:proximal} is given by
\begin{equation}
    \bold v^* = 
\begin{cases}
 \begin{array}{cl}
    \frac{1}{\lambda}\left(1- \frac{1}{\|\bold A^T\bold b\|_2}\right)\bold A^T\bold b &   \|\bold A^T \bold b\|_2 > 1\\
     \bold 0 &  \|\bold A^T\bold b\|_2 \leq 1
 \end{array}
\end{cases}
\label{eq:corollary_condition}
\end{equation}
\end{corollary}

% \begin{corollary}
% The minimizer $\bold v^*$ is given by
% \begin{equation}
%     \bold v^* = 
% \begin{cases}
%  \begin{array}{cl}
%     \left(\bold A^T \bold A + \sfrac{1}{k} \bold I\right)^{-1} \bold A^T \bold b &   \|\bold A^T \bold b\|_2 > 1\\
%      \bold 0 &  \|\bold A^T\bold b\|_2 \leq 1
%  \end{array}
% \end{cases}
% \label{eq:corollary2_condition}
% \end{equation}
% where $k>0$ is the solution to
% \begin{equation}
%     \|\left(k\bold A^T \bold A + \bold I\right)^{-1} \bold A^T \bold b\|_2^2 = 1,
% \end{equation}
% \end{corollary}

% Thus, we have a nice characterization of the solution for special cases, such as when $\bold A$ is orthogonal (in which (\ref{eq:corollary_condition}) holds independent of $\bold b$). In general, we only need to find $k$, which requires solving a polynomial with one variable. A closed-form expression for $k$ may be possible.

% Note that the convergence rate of proximal gradient descent is $O(1/k)$, accelerated proximal gradient descent is $O(1/k^2)$ \cite{parikh2014proximal}, which are both faster and more robust than subgradient descent.
